A Universal Scheme for Dynamic Partitioned Shortest Path Index: Survey, Improvement, and Experiments

Shortest Path (SP) computation is a fundamental operation in many real-life applications such as navigation on road networks, link analysis on social networks, etc. These networks tend to be massive, and graph partitioning is commonly leveraged to scale up the SP algorithms. However, the Partitioned Shortest Path (PSP) index has never been systematically investigated. Moreover, few studies have explored its index maintenance in dynamic networks. In this paper, we survey the dynamic PSP index and propose a universal scheme for its design and analysis. Specifically, we first review the SP algorithms and put forward a novel structure-based partition method classification to facilitate the selection of partition methods. Furthermore, we summarize the existing Pre-boundary PSP strategy and propose two novel strategies (No-boundary and Post-boundary) to improve its index performance. Lastly, we propose a universal scheme with three dimensions (SP algorithm, partition method, and PSP strategy) to facilitate the analysis and design of the PSP index. Based on this scheme, we put forward five new PSP indexes with a prominent query or update efficiency performance. Extensive experiments are conducted to evaluate the performance of the PSP index and the effectiveness of the proposed techniques, with valuable guidance on the PSP index design.

==> RelatedWork.tex <==
\section{Existing PSP Indexes}
\label{sec:ExistingPSP}

%In this section, we first summarize the \textit{graph partition methods} and \textit{SP algorithms}, and then discuss the existing \textit{PSP algorithms}.
% There are three lines of researches that are germane to this research: graph partition methods, shortest path algorithms and partitioned shortest path index.

%It should be noted that although they are integrated with different algorithms, we abstract them as an independent dimension that can be switched interchangeably depending on the different scenarios.

% \subsection{Partitioned Shortest Path Index}

%There are three streams of partition-based shortest path methods depending on the underlying path techniques: 

%\subsection{Graph Partition Methods}
%\label{subsec:graph partition}
%We briefly review the graph partition methods by dividing them into two categories:
%1) Edge-cut Partitioning. 
%Firstly, the \textit{Flow-based Partitioning} (\textit{KaHyPar} \cite{kappa2010, sanders2011engineering}, \textit{PUNCH} \cite{PUNCH11}) utilizes \textit{max-flow min-cut} \cite{ford1956maximal} to split a graph into two parts but cannot achieve balancedness. In particular, \textit{PUNCH} utilizes the \textit{natural cut} heuristics in road networks to achieve high partition quality. Secondly, \textit{Multilevel Graph Partitioning} \cite{barnard1994fast, HL95} such as \textit{SCOTCH} \cite{pellegrini1996scotch} and \textit{METIS}~\cite{Karypis98MeTis} are widely used due to their high efficiency and good partition quality. Besides, it is used as the underlying partitioning algorithm of hierarchical partitions like \textit{HiTi} \cite{jung1996hiti,jung2002efficient}, \textit{SHARC} and \textit{G-Tree} \cite{zhong2013g,zhong2015g,li2019g}. %For example, \textit{HiTi} \cite{jung1996hiti,jung2002efficient} and \textit{SHARC} \cite{bauer2010sharc} organize partitions in \textit{bottom-up} manner by decomposing the original graph into partitions as the lowest level and generates the higher levels recursively by clustering the partitions within the current level. By contrast, \textit{G-Tree} \cite{zhong2013g,zhong2015g,li2019g} organize partitions in \textit{top-down} manner by taking the whole graph as the root on the top level and generate the lower levels by recursively decomposing each partition in the current level. 
%Finally, we also investigated into many other categories of methods like \textit{Spectral Partitioning} \cite{Pothen90SB,barnard1994fast}, 
%There are many \textit{edge-cut partitioning} methods. 
%\textit{Spectral Partitioning} \cite{Pothen90SB,barnard1994fast}, \textit{Graph Growing Partitioning} \cite{goehring1994heuristic,bulucc2016recent} \textit{Bubble}~\cite{diekmann2000shape,schamberger2004partitioning,meyerhenke2006accelerating}), \textit{Geometric Partitioning}
%\cite{BB87RCB,simon1991partitioning,gilbert1998geometric,huang1996effective,schloegel2000graph}, \textit{Minimum $k$-cut} \cite{Saran95,guttmann2000approximation,Goldschmidt94,karger1996new,thorup2008minimum}, \textit{Kernighan–Lin (KL)} \cite{KernighanLin70}, and \textit{Fiduccia-Mattheyses} \cite{FiducciaMattheyses82}. However, their results perform poorly on the PSP algorithms.
%2) Vertex-cut Partitioning.
%It is more effective for graphs with \textit{power-law} distribution \cite{gonzalez2012powergraph,gonzalez2014graphx,roy2015chaos}. 
% We discuss them in two categories: \textit{Online Streaming} and \textit{In-Memory}.
% Intuitively, the \textit{In-Memory} has higher quality since it has complete information.
%The \textit{Online Streaming Algorithms} are widely used for its high efficiency and low memory in distributed systems such as \textit{PowerGraph}~\cite{gonzalez2012powergraph}, \textit{GraphX}~\cite{gonzalez2014graphx}, \textit{Chaos}~\cite{roy2015chaos}, and \textit{HDRF} \cite{petroni2015hdrf}. %\cite{gonzalez2012powergraph} %randomly assigns edges to a partition based on hashing, which 
%They are super-fast but has low quality with high replication. Among them, \textit{CLUGP} \cite{kong2022clustering} performs best by transforming vertex streaming clustering to edge streaming partitioning. 
% \textit{Degree-based Hashing} \cite{xie2014distributed} cuts higher-degree vertices heuristically to reduce the replication factor.  
%\textit{HDRF} \cite{petroni2015hdrf} preserves the locality of low-degree vertices by explicitly cutting the high-degree vertices first. \textit{CLUGP} \cite{kong2022clustering} transforms vertex streaming clustering to edge streaming partitioning. 
%The \textit{In-Memory Algorithms} like \textit{NE} \cite{zhang2017graph,hanai12distributed}, \textit{SMOG} \cite{holzer2009engineering}, \textit{ROAD}~\cite{lee2009fast,lee2010road} usually have much higher partition quality but slow to run. \textit{HEP} \cite{mayer2021hybrid} combines \textit{NE++} and the online \textit{HDRF} for both high quality and efficiency.
%\textit{Neighbor Expansion (NE)} \cite{zhang2017graph} decreases the replication factor by greedily maximizing edge locality. 
%\textit{Neighbor Expansion (NE)} \cite{zhang2017graph} is a famous \textit{in-memory vertex-cut partitioning} method which decreases the replication factor by greedily maximizing edge locality. 
% It iteratively expands a new vertex and all its adjacent edges by minimizing the boundary set. 
%Its distributed version can handle trillion-edge graphs \cite{hanai12distributed}. 
%\textit{HEP} \cite{mayer2021hybrid} combines \textit{NE++} and the online \textit{HDRF}.
%\textit{Shortest-path Multilevel Overlay Graph (SMOG)} \cite{holzer2009engineering} is a hierarchical vertex-separator method which organizes the partitions \textit{bottom-up}. 
% Its multilevel overlay graph is constructed by connecting the separator vertices between adjacent-level graphs through the \textit{upward edges} and \textit{downward edges}. 
%By contrast, \textit{ROAD}~\cite{lee2009fast,lee2010road} builds hierarchical partitions \textit{top-down} by \textit{geometric} \cite{huang1996effective} and \textit{KL} \cite{KernighanLin70}.

%\subsection{Shortest Path Algorithms}
%\label{subsec:Related_SPIndex}
%We summarize the shortest path algorithms that can be used as the building block for partition-based shortest distance indexes: 
%In this section, we summarize the shortest path algorithms that have been used in the existing partition-based indexes: 
%We summarize the shortest path algorithms as follows:

% \noindent 
%1) Direct Search such as \textit{Dijkstra}'s \cite{dijkstra1959note} and $A^*$ \cite{hart1968formal} searches the graph when the index cannot be 
%constructed due to the large graph size (\textit{QbS} \cite{wang2021query}, \textit{ParDist} \cite{chondrogiannis2016pardisp}) or complicated problem (\textit{COLA} \cite{wang2016effective}). %%Nevertheless, s5It takes no time in index update, but %%slowest to 
%queries are slowest;
% \noindent 
%2) Contraction Hierarchy (CH) \cite{geisberger2008contraction} is a widely used lightweight index that contracts the vertices in a pre-defined order and preserves the shortest path information by adding shortcuts among the contracted vertex's neighbors. 
%The \textit{search-based CH} \cite{geisberger2008contraction} has a small index size but takes longer to build and maintain \cite{zhang2021experimental,geisberger2012exact} while \textit{concatenation-based CH} \cite{ouyang2020efficient,wei2020architecture} is much faster to build and maintain if the tree-width is small.
% When using search-based construction \cite{geisberger2008contraction} it has smaller sizes, but takes longer to build and maintain \cite{zhang2021experimental,geisberger2012exact}; when using concatenation-based construction \cite{ouyang2020efficient,wei2020architecture}, it is much faster to build and maintain if the tree-width is small. 
%\textit{CH}'s query performance is generally around 10$\times$ faster than the \textit{direct search} but much slower than the \textit{hub labelings}. Surprisingly, no PSP index has used \textit{CH} as underlying index;
% \noindent 
%3) Pruned Landmark Labeling (PLL). Although many \textit{hub labeling} methods have been proposed in the past decade, only two are widely used. Built by either \textit{pruned search} \cite{akiba2013fast} or \textit{propagation} \cite{li2019scaling,jin2020parallelizing,zhang2021efficient,zhang2023parallel}, \textit{PLL} is the only index that can work on the graph with large treewidth. Therefore, graphs with this property use it as the underlying index (\eg \textit{QsB} \cite{wang2021query,farhan2022batchhl} for its landmarks, \textit{CT-Index} \cite{li2020scaling,zheng2022workload} for its core);
% \noindent 
%4) Tree Decomposition (TD)\cite{ouyang2018hierarchy,chang2012exact,wei2012tedi,chen2021p2h,zhang2021dynamic}. As another widely used hop labeling, it is much faster than \textit{PLL} for graphs with smaller treewidth but cannot scale to large ones. For instance, \textit{CT-Index} \cite{li2020scaling,zheng2022workload} uses it for its periphery, and \textit{FHL} \cite{liu2021efficient,liu2022FHL} use it as a forest;
% \noindent 
%5) All Pair Pre-computation pre-computes all-pair distance with the fastest query, but incurs long index construction and large index storage. \textit{G-Tree} \cite{zhong2013g,zhong2015g} and \textit{ROAD} \cite{lee2009fast,lee2010road} store the distance between boundary vertices in each partition.


%\subsection{Partitioned Shortest Path Algorithms}
%\label{subsec:PartitionedSP}
%Recently, multiple surveys about the SP computation have emerged, focusing 
There are several SP surveys on transportation networks \cite{bast2016route}, complex networks \cite{zhang2022shortest}, static \cite{madkour2017survey, li2017experimental, wu2012shortest}, and dynamic graphs \cite{zhang2021experimental}, but none considers the partitioned scenario. The PSP framework is proposed in \cite{chondrogiannis2014exploring, chondrogiannis2016pardisp}, but its dynamic version is not discussed. %In this work, we study the dynamic PSP problem systematically and explore its performance in both road networks and complex networks by involving the SOTA SP algorithms and partition methods. Specifically, 
In the following, we discuss and categorize the existing \textit{PSP} methods based on our scheme: %\newline 
1) Pre-Boundary + Search/All-Pair + Hierarchy/ Planar: \textit{HiTi} \cite{jung2002efficient}, \textit{Graph Separators}, \textit{CRP} \cite{delling2017customizable} \cite{holzer2009engineering}, \textit{ParDiSP} \cite{chondrogiannis2014exploring,chondrogiannis2016pardisp} pre-compute  shortest distances between boundaries to guide the search. In a broad sense, \textit{Arc-flag} \cite{mohring2007partitioning} and \textit{SHARC} \cite{bauer2010sharc} also belong to this category. \textit{G-tree} \cite{Gtree_zhong2013g,Gstar_tree_li2019g} uses dynamic programming to compute the distance between layer's all-pair information to replace searching and it is used in \textit{kNN} \cite{zhong2015g}, \textit{ride-sharing} \cite{ta2017efficient}, \textit{time-dependent} \cite{wang2019querying}, and \textit{distance embedding} \cite{huang2021learning}. They are slow to construct due to \textit{Pre-B} and inefficient to query due to direct search; %\newline
2) Pre-Boundary+Search/PLL+Planar: 
\textit{COLA} \cite{wang2016effective} builds labels for the \textit{skyline shortest path} on the overlay graph for the constrained shortest path. Its construction suffers from \textit{Pre-B} and query suffers from searching; %\newline
3) Pre-Boundary+TD/TD+Planar: \textit{FHL} \cite{liu2021efficient,liu2022FHL} builds the \textit{TD} both within and between partitions for multi-dimensional skyline paths. %As validated in Exp 4, our \textit{Post-B} can speedup \textit{Pre-B}'s construction dramatically; %\newline 
4) Pre-Boundary+PLL/PLL+Planar: \textit{T2Hop} \cite{li2019time,li2020fastest} utilizes two layers of \textit{PLL} to reduce the complexity of long-range time-dependent paths, and this structure's performance is limited by \textit{PLL}; %\newline 
5) No-Boundary+ PLL/TD+Core: \textit{Core-Tree} \cite{CT_li2020scaling,zheng2022workload,DCT_zhou2024Scalable} is the baseline we discussed; 
6) Pre-Boundary+Search/All-Pair/PLL+Sketch: This category works on huge graphs where index is impossible so only a small number of landmarks are selected to prune the search \cite{das2010sketch,wang2021query,farhan2022batchhl} or approximate the result \cite{gubichev2010fast,qiao2012approximate}. %In summary, %%Therefore, 
%all the existing \textit{PSP} methods have their limitation, warranting %%and it is worthwhile to 
%the comprehensive investigation embarked on %%as %%e the \textit{PSP} problem 
%in this paper.


%However,[the weakness of existing works]
